Scalable Network Tomography for Dynamic Spectrum Access

Mobile networks have increased spectral efficiency through advanced multiplexing strategies that are coordinated by base stations (BS) in licensed spectrum. However, external interference on clients leads to significant performance degradation during dynamic (unlicensed) spectrum access (DSA). We introduce the notion of network tomography for DSA, whereby clients are transformed into spectrum sensors, whose joint access statistics are measured and used to account for interfering sources. Albeit promising, performing such tomography naively incurs an impractical overhead that scales exponentially with the multiplexing order of the strategies deployed -- which will only continue to grow with 5G/6G technologies. To this end, we propose a novel, scalable network tomography framework called NeTo-X that estimates joint client access statistics with just linear overhead, and forms a blue-print of the interference, thus enabling efficient DSA for future networks. NeTo-X's design incorporates intelligent algorithms that leverage multi-channel diversity and the spatial locality of interference impact on clients to accurately estimate the desired interference statistics from just pair-wise measurements of its clients. The merits of its framework are showcased in the context of resource management and jammer localization applications, where its performance significantly outperforms baseline approaches and closely approximates optimal performance at a scalable overhead.

==> motivation.tex <==
\section{HOD as a Core Primitive}
\label{sec:motivation}

\subsection{Motivation}
%\karthik{Include results for HTs, multiple antennas and channels, compare to Oracle instead of SP}
\begin{figure}
    \begin{subfigure}[b]{0.35\linewidth}
    \captionsetup{justification=centering}
        \centering
        \includegraphics[width=\textwidth]{plots/Motivation-HT-n.pdf}
        % \caption{Four-channel, 30 client, SISO system}
        \caption{SISO}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.64\linewidth}
    \captionsetup{justification=centering}
        \centering
        \includegraphics[width=\textwidth]{plots/Motivation-MIMO.pdf}
        % \caption{Four-channel, 30 client, \newline MU-MIMO system}
        \caption{MU-MIMO}
    \end{subfigure}
    \caption{HOD prevents drop in performance with (a) increased interference, (b) larger number of antennas}
    \label{fig:motivation}
\end{figure}
% \karthik{Illustration to explain problem and setting}

We first motivate the need for estimating high-order channel access distributions (HOD) of clients. Unlike an asynchronous WiFi network, a synchronous cellular network enables BSs to centrally schedule both its DL and UL transmissions.  This tight control enables the high multiplexing gains offered by 5G antenna technologies. However, in an open/unlicensed spectrum, the presence of HTs cause external interference, which affects clients, but cannot be sensed by the BSs through LBT (shown in Fig.~\ref{fig:HT-channel}).  
%\karthik{Readers might not know about LBT. So I added one line}
%\karthik{Refer to an existing LBT work. LBT was not mentioned anywhere before.}
This causes centralized scheduling to become a major drawback, and severely affects the network's multiplexing ability. We conduct network simulations (details in Sec.~\ref{sec:eval}) with a single LTE BS, several tens of clients and a variable number of interfering sources, to highlight this impact. The conventional proportional fair (PF) scheduler~\cite{kushner_convergence_2004} is employed at the BS. The results presented in Fig.~\ref{fig:motivation} reveal three key observations: 

(i) {\em Interference impact is significant:} As the number of HTs increases, the  ability of the BS to deliver or receive traffic from the affected clients diminishes, leading to a rapid drop in resource utilization with just a few HTs, as seen in Fig.~\ref{fig:motivation}(a). This reveals existing networks' acute vulnerability to interference. 

(ii) {\em Limited interference information is useful, but not sufficient:} 
In contrast to PF which is interference-agnostic, we consider an alternate {\em access-aware} (AA) scheme. It incorporates some knowledge of the interference---namely the probability that individual clients can access the channel---to weigh the clients' utility in the scheduling decisions. We consider both SISO and MU-MIMO performance in Figs.~\ref{fig:motivation}(a) and (b) respectively. The AA scheme performs 50-100\% better than PF, which is promising.

However, as more antennas $M$ are introduced in our 5G systems, the throughput depends on the specific set of users that are jointly scheduled on the same resource. Hence, in addition to the access probabilities of `individual' clients considered in AA, we also consider an Oracle scheduling scheme that has access to all higher order `joint' access distributions of all combinations of clients (limited by $M$). Figs.~\ref{fig:motivation}(a) and (b) reveal that while AA improves performance, there is still a wide gap to the theoretical performance that is possible with HODs. 

% \karthik{Why does PF grow linearly with antennas even in the presence of interference in Fig.1b.}
% (iii) {\em HOD are essential to retain multiplexing gain in MU-MIMO systems:}The MU-MIMO version of the PF and AA schedulers do not consider the ability of the clients selected to `simultaneously' use the resources in the presence of interference. Hence, as the multiplexing order ($M$) increases in Fig.~\ref{fig:motivation}(b), this has an even greater impact(compared to the SISO system), severely limiting the multiplexing gain that could be achieved, as is observed with respect to Oracle's performance -- the latter benefiting from interference-aware `group' selection that is critical for MU-MIMO, and made possible by HOD.

(iii) {\em HODs useful even in SISO systems:}
In a SISO system, why might we need access to the HOD?  With only a single antenna, shouldn't the individual channel access (AA) be enough? 
% Note, however, that in an AA scheme, the BS employs first-order  access probabilities of clients to `hedge' the risk of interference, when scheduling its resources.  
Consider, however, that in AA, once a client is scheduled, it is possible for the allocated resources to be completely wasted if there is interference at the client. Having access to HODs, allows the Oracle to speculatively \textit{over}-schedule multiple clients (on the UL) on the \textit{same}, single antenna resource.  By using the HOD it intelligently selects clients so as to maximize the expected resource utilization over time while minimizing the probability of collisions. This results in a much more graceful degradation in the Oracle's performance with increasing interference, compared to AA in the SISO system in Fig.~\ref{fig:motivation}(a). We discuss this approach in Sec.~\ref{sec:sched_sp}. 

\begin{comment}
Once the resources are allocated, however, we still risk wasting them entirely in the event that the scheduled UE is interfered with because only one UE is scheduled per resource.  The key result from our previous work was to speculatively \emph{overschedule} resources in such away to further mitigate this risk of wasted wireless resources.  Previously, we relied on a heuristic to perform this speculative scheduling, but ideally the BS could simply scale the AA scheme to incorporate the full joint channel access distribution.  Doing so allows us to optimally schedule multiple clients simultaneously.

by first discussing it in the context of mobile network (e.g. LTE, 5G) scheduling in unlicensed spectrum (e.g. Wi-Fi)\footnote{We emphasize that the technique is general enough to be applied to multiple applications, e.g. the task of localizing interferers which will be discussed later.} for both single- (SISO) and multi-antenna systems (MIMO.  We consider the fact that the Wi-Fi nodes are HTs relative to the central base station (BS) of the mobile network.  That is, their use of the spectrum interferes with the mobile network end user equipment (UEs) but their transmissions cannot be sensed by the BS.  This interference will cause a drop in the total network throughput as the BS schedules flows and attempts to deliver or receive traffic from the affected UEs, wasting network resources.

\emph{SISO} Fig.~ \ref{fig:motivation}a shows the performance of three scheduling schemes in the presence of this kind of interference.  We simulate the total network throughput of a SISO system with UEs operating in the presence of increasing numbers of HTs.
%PF
A typical implementation of proportional fair (PF) scheduling does not consider the impact of interference in the network, and thus suffers the most from an increase in the number of HTs.  
%AA
A better approach which we call access aware (AA), is to incorporate some knowledge of the interference into the scheduling algorithm.  Assume that the BS has an estimate of the probability each client can access the channel, i.e. the probability that each user will \emph{not} be interfered with by a HT.  Then we can then use this probability as a weight when prioritizing the schedule.  The AA scheme performs 50-100\% better than PF.
% SP
% OVERscheduling is even better
The improvement of AA over PF demonstrates the utility in knowledge of the channel access distribution to improving the scheduling scheme.  We can do better, though.  In the AA scheme the BS has the first-order marginal channel access probabilities, which it uses to ``hedge" the risk of interference when scheduling the wireless resources.  Once the resources are allocated, however, we still risk wasting them entirely in the event that the scheduled UE is interfered with because only one UE is scheduled per resource.  The key result from our previous work was to speculatively \emph{overschedule} resources in such away to further mitigate this risk of wasted wireless resources.  Previously, we relied on a heuristic to perform this speculative scheduling, but ideally the BS could simply scale the AA scheme to incorporate the full joint channel access distribution.  Doing so allows us to optimally schedule multiple clients simultaneously.

% MIMO
\emph{MIMO} Knowledge of the interference HOD is not only useful in SISO systems.
Scheduling in multi-user (MU-MIMO) and massive MIMO systems involves not only allocating resource blocks to UEs, but choosing which set of multiple UEs to serve simultaneously.
\hl{The MIMO version of the PF scheduler picks sets of UEs based only on the maximum utility.  It is unaware of the interference, so it doesn't consider whether or not the UEs that it picks will be able to use the resources.
This mismatch has an even greater impact than in the SISO system because it severely limits the multiplexing gain that could be achieved.
\textbf{Is this accurate?}
}
5G systems increase overall network throughput by serving multiple users simultaneously via many antennas, but they are not designed with interference in mind.  A naive application of existing scheduling methods in the presence of interference nullifies any multiplexing gains delivered by the additional antennas.  
Fig.~\ref{fig:motivation}b demonstrates how partial (AA) and full knowledge of the HOD improves the cumulative network throughput of MIMO scheduling.  Again, we see that some knowledge of the interference pattern is useful, but it doesn't approach the theoretical performance of using the HOD.

% challenges in scaling -> need for our approach

% Mobile networks have expanded to support a number of technologies using the same spectrum resources. Quite often this leads to substantial interference on crowded channels which hurts the performance of uninformed and non-adaptive schedulers as seen in Fig.~ \ref{fig:HT-plt}. In a standard implementation of proportional fair (PF) scheduling, due to increased occupancy of the channel resources, throughputs drop to substantially low numbers. Having an access-aware (AA) scheme which scales the priority queue to better suit the channel dynamics tends to improve the performance by a margin of ~50-100\%. Having restricted information about the network can only take us so far. However, knowledge of the HTs dynamics and their impact on the clients reveals another dimension to the gains that could possibly be achieved. Introduction of speculative (SP) scheduler, which relies on an intelligent mechanism of estimating higher-order marginals with scalable measurements,  helps to overshedule clients and utilize resource blocks with significantly better efficiency. This leads to gains of another ~50-100\% \textit{over} access-aware (AA) in high contention environments.

\end{comment}

\subsection{Challenges}
While HODs enables a network to operate in a smarter, more efficient way, the challenge lies in acquiring them in the first place.
Since the interference is hidden from the BS,
we rely on the clients to act as sensors and estimate their local interference. %on their own.
However, such an approach would reveal only the first-order \emph{marginal} probabilities, i.e. ``What is the probability that client $i$ is interfered with?"  
We have seen (Fig.~\ref{fig:motivation}) that we require 
the HOD to operate the network efficiently.  The HOD answer questions such as ``What is the probability that client $i$ is interfered with but clients $j$ and $k$ are not?"
We could continue to measure the HOD directly by scheduling each possible combination of clients and observing the results, but in an $M$-antenna MU-MIMO system with $N$ total clients, this results in an exponential measurement overhead ($O(2^M)$) which affects the resources available for data transfer. Note that, if the system employs multiple channels ($C$), as is the common case today with carrier aggregation~\cite{CA}, then this overhead further scales as $O(C\cdot 2^M)$.   
%How would one go about measuring these probabilities?  The number of measurements required is obviously a function of the number of users served by the network, but also the number of antennas and the number of channels.  As each of these parameters increases, so to does the number of measurements required to accurately estimate the desired probability.
Fig.~\ref{fig:motivation}(b) demonstrates this challenge by plotting the number of measurements required to estimate the desired HOD for an increasing number of antennas.  While the AA scheme does not rely on HODs, %the number of measurements does not increase with the number of antennas.  On the other hand, 
the number of measurements needed by the \textit{oracle} to estimate and benefit from HOD increases exponentially, making it impractical.

To address this fundamental challenge, our proposed a network tomography approach for DSA, \system, allows us to leverage the benefits of HODs, not just for scalable performance in higher-order antenna and channel systems, but also in other interference-analysis applications (e.g. jammer localization)---all at a practical overhead that scales linearly with the number of channels employed and the clients ($O(C \cdot N + C\cdot {K \choose 2})$). 
% \karthik{make it consistent with intro}

\begin{comment}
    

With knowledge of an HOD, a network can operate in a smarter and more efficient way, the challenge is of course in acquiring that knowledge in the first place.  The first challenge is that the interference is by definition \emph{hidden} from the BS.  The solution here is easy enough--employ the distributed users as sensors to their own, locally occuring interference. 

The second challenge is that this only tells us about first degree \emph{marginal} probabilities, i.e. ``What is the probability that user $i$ is interfered with?"  As seen in Fig.~\ref{fig:motivation} we need higher order distributions to operate the network efficiently, e.g. ``What is the probability that user $i$ is interfered with but user $j$ is not?"
How would one go about measuring these probabilities?  The number of measurements required is obviously a function of the number of users served by the network, but also the number of antennas and the number of channels.  As each of these parameters increases, so to does the number of measurements required to accurately estimate the desired probability.

Fig.~\ref{fig:motivation}(b) demonstrates this challenge by plotting the number of measurements required to estimate the \hl{desired distribution FIXME} for an increasing number of antennas.  Because the AA aware scheme does not rely on the HOD, the number of measurements does not increase with the number of antennas.  On the other hand, the theoretical number of measurements to get the \hl{desired HOD} increases exponentially.



\karthik{Interference-awareness helps -- AA, but need HOD for scalable benefits -- Oracle; hence, need HOD}
 \karthik{simple numerical result on why obtaining HOD is not scalable with multiple channels, antennas}

% \% If you could obtain HOD and blue-print (BP) interference dependencies across clients, how can it benefit?
%  (resource management for better spectral efficiency, load balancing and effective carrier aggregation, localizing clients and jammers/interferers, anything else? )

% \% What are the technical challenges in obtaining HOD and BP interference?
%  (Overhead, impact of wrong estimates/decisions, environment/client dynamics/mobility, anything else?)
%  Is there a way to formalize the problem?

\end{comment}
